Minding Language Models' (Lack of) Theory of Mind: A Plug-and-Play Multi-Character Belief Tracker

Theory of Mind (ToM)$\unicode{x2014}$the ability to reason about the mental states of other people$\unicode{x2014}$is a key element of our social intelligence. Yet, despite their ever more impressive performance, large-scale neural language models still lack basic theory of mind capabilities out-of-the-box. We posit that simply scaling up models will not imbue them with theory of mind due to the inherently symbolic and implicit nature of the phenomenon, and instead investigate an alternative: can we design a decoding-time algorithm that enhances theory of mind of off-the-shelf neural language models without explicit supervision? We present SymbolicToM, a plug-and-play approach to reason about the belief states of multiple characters in reading comprehension tasks via explicit symbolic representation. More concretely, our approach tracks each entity's beliefs, their estimation of other entities' beliefs, and higher-order levels of reasoning, all through graphical representations, allowing for more precise and interpretable reasoning than previous approaches. Empirical results on the well-known ToMi benchmark (Le et al., 2019) demonstrate that SymbolicToM dramatically enhances off-the-shelf neural networks' theory of mind in a zero-shot setting while showing robust out-of-distribution performance compared to supervised baselines. Our work also reveals spurious patterns in existing theory of mind benchmarks, emphasizing the importance of out-of-distribution evaluation and methods that do not overfit a particular dataset.

==> sections/fundamental_challenges_datasets.tex <==
\section{Fundamental Challenges of Existing ToM Datasets}
A widely adopted test for assessing children's social cognitive ability to reason about others' mental states is the Sally-Anne test \citep{wimmer1983beliefs, baron1985does} (Figure \ref{fig1:tom_example} shows an example of the Sally-Anne test).
Inspired by this test, two NLP datasets were developed: ToM-bAbi \citep{nematzadeh2018evaluating}, and then ToMi \citep{le2019revisiting}, expanding on the former. Similar to bAbI \citep{weston2015towards}, ToMi automatically generates a short story involving two or three characters, and then evaluates a model's reasoning capabilities through question answering. ToMi expands on ToM-bAbI, introducing one distractor sentence and one distractor character, plus allowing more flexibility in the event sequences. Still, both datasets follow the plot of the original Sally-Anne test: $A$ and $B$ are in a room, and $A$ moves an object from an opaque container to another. $B$ may or may not leave the room before $A$ moves the object. $B$ will know the new object's location if and only if they were in the room at the time of the movement. Then, four types of ToM questions are posed: first-order and second-order ToM questions, that can probe a character about either a false-belief or a true-belief they hold (i.e, belief that matches reality). Additionally, ToMi includes a question probing about reality (or zeroth-order ToM) and memory.

ToMi has six types of sentences, which we will refer to as \textit{primitives}. Despite the limited types of primitives, stories may require high-order levels of reasoning to correctly answer the probing questions. Each primitive has one sole way of phrasing each sentence. The primitives are: someone enters or exits a room; the location of an object or a person; someone moved an object; someone likes or hates an object (distractor sentence). In ToM-bAbI and ToMi all object names, containers, rooms, and characters' names are sampled uniformly from a list of manually selected strings. This often causes violations of physical commonsense, among other issues we will discuss next.

\subsection{Fixing Accidentally Ambiguity and 3-hop Reasoning Tasks in ToMi}

\begin{table}[t]
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{l}
        \hline
1. Jacob entered the front yard. \\
2. Lucas entered the front yard. \\ 
3. Hunter entered the kitchen. \\
4. The eggplant is in the suitcase. \\ 
5. Lucas exited the front yard. \\ 
6. Lucas entered the kitchen. \\ 
7. Jacob moved the eggplant to
the \textbf{pantry}. \\
8. Where will Lucas look for the eggplant? \\ 
\hline
       \end{tabular}
       \caption{ToMi sample where the second object container is a pantry. Since pantries are usually located in kitchens and not in front yards, readers may assume Lucas saw Jacob storing the eggplant.\\}
       \label{tab:example1}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{l}
        \hline
1. Jacob entered the front yard. \\
2. Lucas entered the front yard. \\ 
3. Hunter entered the kitchen. \\
4. The eggplant is in the suitcase. \\ 
5. Lucas exited the front yard. \\ 
6. Lucas entered the kitchen. \\ 
7. Jacob moved the eggplant to
the \textbf{bottle}. \\
8. Where will Lucas look for the eggplant? \\ 
\hline
        \end{tabular}
        \caption{ToMi sample where the second object container is a bottle. Readers may assume the bottle is in the front yard since there was no further specification -- therefore concluding Lucas did not observe the movement.\\}
        \label{tab:week2}
     \end{subtable}
     \caption{Two samples from the ToMi dataset, only differing in the highlighted noun. In ToMi, objects, containers, and rooms are selected randomly from a specified list. In both cases, the expected response in ToMi is \textit{suitcase}. Humans nonetheless assume different underlying scenarios, guided by physical commonsense.}
     \label{table:tomi-two-examples}
\end{table}

ToMi is automatically generated, and uniformly samples among a list of all possible objects, locations, containers, and rooms, to create the final stories. The assumption is that no matter the noun selection, the underlying answers will be the same. Qualitative analysis shows this assumption may be incorrect if physical commonsense leads humans to assume other interpretations. Table \ref{table:tomi-two-examples} shows two ToMi samples, where in the first case readers will likely assume that an entity changed rooms (which never occurs in ToMi).

In some cases, ToMi's unintentional ambiguity may be resolved at a later step in the story (see \citep{arodi-cheung-2021-textual-time}. Supervised models will overfit to ToMi's assumptions, and thus off-the-shelf approaches will not be fairly compared.

In all cases, lack of physical commonsense adds 3-hop reasoning abilities to succeed in ToMi, which convolutes measuring Theory of Mind skills and was not the original authors' intent. Concretely, in Table \ref{table:tomi-two-examples}b, the reader needs to conclude from \texttt{``Jacob is in front yard'', ``eggplant is in suitcase'' and ``Jacob moved the eggplant''} that the suitcase is in the front yard, and hence Lucas saw it there. To fix ambiguities and accidental 3-hop reasoning tasks, and instead solely measure Theory of Mind reasoning skills, we automatically add a sentence describing the location of each container (e.g., \texttt{``The suitcase is in the front yard''}. Since ToMi is itself automatically generated, this involves only subtly modifying the generator script. From now onwards, ``ToMi'' refers to ToMi with the disambiguation sentence addition.

Following \citet{arodi-cheung-2021-textual-time,sap2022neural}, in addition to this solution for unintentional ambiguity, we also correct mislabeled second-order questions.


==> sections/fundamental_challenges_datasets_v2.tex <==
\section{Fundamental Issues in Existing ToM Datasets}

% As introduced in \S\ref{sec:motivation}, 
\editmel{As introduced in \S\ref{sec:motivation}}, 
the sole large-scale theory of mind dataset for reading comprehension tasks is ToMi \citep{le2019revisiting}. %\footnote{As reported in \citet{arodi-cheung-2021-textual-time,sap2022neural}, ToMi contains some mislabeled second-order questions, which we correct in our experiments. } 
Barring its added distractor characters and sentences, ToMi strictly mimics the Sally-Anne test, a widely adopted evaluation for assessing children's social cognitive ability to reason about others' mental states \citep{wimmer1983beliefs, baron1985does}. 
Stories are structured are as follows: characters $A$ and $B$ are in a room, and $A$ moves an object from an opaque container to another; $B$ may or may not leave the room before $A$ moves the object. 
$B$ will know the object's new location if and only if they were in the room at the time it was moved. 
Four types of ToM questions are posed: first-order or second-order, probing a character about either a true or a false belief (i.e, belief that matches reality or not). 
ToMi also includes questions probing about reality~\citep[or \textit{zeroth-order} ToM,  ][]{sclar22symmetric} and memory.

ToMi has six types of sentences (i.e. six \textit{primitives}) with \editmel{set} phrasing. These include: someone (a) entering or (b) exiting a room; the location of (c) an object or (d) a person; (e) someone moving an object; and (f) someone's opinion about an object (distractors). %\footnote{Sentences generated from (f) serve as distractors.} 
Primitives are combined into stories with a finite list of possible orderings. Despite the limited types of primitives, the resulting stories require high-order levels of reasoning to correctly answer the posed questions. 
Finally, templated stories are filled with randomly sampled objects, locations, containers, and rooms from a set list.


%ToMi includes six types of sentences (i.e. six \textit{primitives}) with templated phrasing.
%These include: someone (a) entering or (b) exiting a room; the location of (c) an object or (d) a person; (e) someone moving an object; and (f) someone's opinion about an object.\footnote{Sentences generated from (f) serve as distractors.}
%Primitives are combined into stories using a finite list of possible orderings.
%Finally, ToMi fills these templated stories with randomly sampled objects, locations, containers, and rooms from a set list. 
%Despite the limited types of primitives, sentence orderings, and entities to fill, the resulting stories require high-order levels of reasoning to correctly answer the posed questions. 

%Each primitive has one sole way of phrasing it. 
% The primitives are: someone enters or exits a room; the location of an object or a person; someone moved an object; someone likes or hates an object (distractors). %All nouns in the story are sampled uniformly from a prefix list. % All object names, containers, rooms, and characters' names are sampled uniformly from a list of manually selected strings. This often causes violations of physical commonsense, among other issues we will discuss next.

%A widely adopted test for assessing children's social cognitive ability to reason about others' mental states is the Sally-Anne test \citep{wimmer1983beliefs, baron1985does} (Figure \ref{fig1:tom_example} shows an example of the Sally-Anne test).
%Inspired by this test, two NLP datasets were developed: ToM-bAbi \citep{nematzadeh2018evaluating}, and then ToMi \citep{le2019revisiting}, expanding on the former. Similar to bAbI \citep{weston2015towards}, ToMi automatically generates a short story involving two or three characters, and then evaluates a model's reasoning capabilities through question answering. ToMi expands on ToM-bAbI, introducing one distractor sentence and one distractor character, plus allowing more flexibility in the event sequences. Still, both datasets follow the plot of the original Sally-Anne test: $A$ and $B$ are in a room, and $A$ moves an object from an opaque container to another. $B$ may or may not leave the room before $A$ moves the object. $B$ will know the new object's location if and only if they were in the room at the time of the movement. Then, four types of ToM questions are posed: first-order and second-order ToM questions, that can probe a character about either a false-belief or a true-belief they hold (i.e, belief that matches reality). Additionally, ToMi includes a question probing about reality (or zeroth-order ToM) and memory.

%\subsection{Fixing Accidentally Ambiguity and 3-hop Reasoning Tasks in ToMi}

\begin{comment}
\begin{table}[t]
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{l}
        \hline
1. Jacob entered the front yard. \\
2. Lucas entered the front yard. \\ 
3. Hunter entered the kitchen. \\
4. The eggplant is in the suitcase. \\ 
5. Lucas exited the front yard. \\ 
6. Lucas entered the kitchen. \\ 
7. Jacob moved the eggplant to
the \textbf{pantry}. \\
8. Where will Lucas look for the eggplant? \\ 
\hline
       \end{tabular}
       \caption{ToMi sample where the second object container is a pantry. Since pantries are usually located in kitchens and not in front yards, readers may assume Lucas saw Jacob storing the eggplant.\\}
       \label{tab:example1}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.45\textwidth}
        \centering
        \begin{tabular}{l}
        \hline
1. Jacob entered the front yard. \\
2. Lucas entered the front yard. \\ 
3. Hunter entered the kitchen. \\
4. The eggplant is in the suitcase. \\ 
5. Lucas exited the front yard. \\ 
6. Lucas entered the kitchen. \\ 
7. Jacob moved the eggplant to
the \textbf{bottle}. \\
8. Where will Lucas look for the eggplant? \\ 
\hline
        \end{tabular}
        \caption{ToMi sample where the second object container is a bottle. Readers may assume the bottle is in the front yard since there was no further specification -- therefore concluding Lucas did not observe the movement.\\}
        \label{tab:week2}
     \end{subtable}
     \caption{Two samples from the ToMi dataset, only differing in the highlighted noun. In ToMi, objects, containers, and rooms are selected randomly from a specified list. In both cases, the expected response in ToMi is \textit{suitcase}. Humans nonetheless assume different underlying scenarios, guided by physical commonsense.}
     \label{table:tomi-two-examples}
\end{table}
\peter{Trying out a new, more compressed version of the table above}
\end{comment}

\begin{table}[t]
\centering
\begin{tabular}{l}
\toprule
\begin{tabular}[l]{@{}l@{}}
1. Oliver entered the front yard. \\
2. Ethan entered the front yard. \\ 
3. Liam entered the kitchen. \\
4. \textbf{objectA} is in the basket. \\ 
5. Ethan exited the front yard. \\ 
6. Ethan entered the kitchen. \\ 
7. Oliver moved \textbf{objectA} to
the \textbf{containerX}. \\
8. Where does Ethan think \textbf{objectA} is? \\
\end{tabular} \\  \midrule
\textit{ToMi Gold Label:} basket \\ \bottomrule
\end{tabular}
\caption{Interpretation of ambiguities in ToMi can be affected by commonsense. 
In the above template, the correct label is that Ethan thinks \textbf{objectA} is in the \textit{basket}, as this is where he last saw it. 
Setting \textbf{objectA} to \emph{hat} and \textbf{containerX} to \emph{box} results in 80\% human accuracy. 
However, setting these to \emph{apple} and \emph{pantry}, accuracy drops to 20\%. 
Physical commonsense suggests the pantry is likely in the kitchen, changing the answer to \emph{pantry}, but regardless of the identity of \textbf{objectA} or \textbf{containerX}, the correct label in ToMi is \emph{basket}. }\label{table:tomi-two-examples}
\end{table}

\paragraph{Addressing Underspecification}
ToMi's story construction process often leaves object locations ambiguous; for example, the location of the \textit{basket} in line 4 of Table~\ref{table:tomi-two-examples}.
This ambiguity is at times resolved by a later sentence in the story~\citep{arodi-cheung-2021-textual-time}, but this resolution happens only infrequently, and such resolutions were not expressly intended by ToMi's original design.
This complicates the task beyond theory of mind.
For example, in Table \ref{table:tomi-two-examples}, the reader must conclude from \textit{``Oliver is in front yard''}, \textit{``Oliver moved the objectA (...)''}, and \textit{``The objectA is in basket''} that the basket is in the front yard, and hence that Ethan saw it there. 
This requires 3-hop reasoning, and knowing ahead of time that, in ToMi, characters do not change rooms unless explicitly stated.

In light of these ambiguities, we find that human readers rely heavily on physical commonsense reasoning to perform reading comprehension.
% This story construction process implicitly assumes that questions about the story do not depend on how the templates are filled, only the underlying story template. 
% However, we find that ToMi's approach to story generation can introduce ambiguity and disagreement among human readers, particularly with respect to physical commonsense reasoning.
% in a small-scale human study we find physical commonsense leads human answers to change, depending on the noun. 
Table \ref{table:tomi-two-examples} presents an example where %human evaluation shows that 
the in-filled object and container have a large effect on human~responses.\footnote{Using Amazon Mechanical Turk, we present 20 humans with the template in Table 1, using either \emph{(hat,box)} or \emph{(apple, pantry)}. Workers are paid \$1 per HIT.} % to assume that an entity changed rooms (which never occurs in ToMi
% , following the Sally-Anne test
%) or not. Supervised models overfit to these
% ToMi's
%assumptions and thus obtain high in-domain performance but fail to generalize to realistic scenarios. 
% have an unfair advantage over other approaches.
% \as{how do we address this / what's the takeaway here? does this just lead to an upper bound in performance?}\mel{the takeaway is that you shouldn't assume that humans (nor self-supervised models) should be able to perform this task without extra clarification -- like adding a sentence}
In certain cases, real human readers disagree with these ToMi labels, which are dependent primarily on the underlying story template and assumptions about character movements, rather than on the objects and associated commonsense reasoning.

% Object locations in ToMi are often left ambiguous
% in many instances of this dataset (see line 4 of Table \ref{table:tomi-two-examples}). 
%, nor was it an expressed intention of the original authors.
% In all cases, lack of physical commonsense adds the requirement to perform 3-hop deductions to succeed in ToMi. 
%This ambiguity convolutes the task which is measuring theory of mind skills and was not the ToMi's authors' intent. 
\editmel{
To solve these unintentional ambiguities and additional 3-hop reasoning requirements, and instead solely measure theory of mind reasoning skills,}
%we use a modified version of ToMi.
% To remove these additional 3-hop reasoning requirements, and instead solely measure theory of mind reasoning skills.
\editmel{we use a modified version ToMi. We}
%We correct this underspecification by 
automatically add a sentence that dismbiguates the location of each container immediately after each primitive (c) or (e) %describing containers 
(e.g., adding \textit{``The basket is in the front yard''} as line 5 in Table \ref{table:tomi-two-examples}). %Since ToMi is automatically generated, this implies only a minor modification to the generator script.
\editmel{Finally, as reported in \citet{arodi-cheung-2021-textual-time,sap2022neural}, ToMi contains some mislabeled second-order questions, which we also correct.} %%% i want to say this in the main text --- it also adds to the idea that the dataset has issues, and we are not the first to say. This was like 20% of the second-order questions, they really were not careful


% \as{I'm not sure this is worth putting in main paper since it's so short and already reported. We could add a footnote in the first par of this section saying we correct these existing identified examples}
%In all experiments, ``ToMi'' refers to ToMi with correctly labeled questions and  disambiguation sentences added. %in addition to this solution for unintentional ambiguity, we also correct mislabeled second-order questions.

